Towards Robust LiDAR-based Perception in Autonomous Driving: General Black-box Adversarial Sensor Attack and Countermeasures

Perception plays a pivotal role in autonomous driving systems, which utilizes onboard sensors like cameras and LiDARs (Light Detection and Ranging) to assess surroundings. Recent studies have demonstrated that LiDAR-based perception is vulnerable to spoofing attacks, in which adversaries spoof a fake vehicle in front of a victim self-driving car by strategically transmitting laser signals to the victim's LiDAR sensor. However, existing attacks suffer from effectiveness and generality limitations. In this work, we perform the first study to explore the general vulnerability of current LiDAR-based perception architectures and discover that the ignored occlusion patterns in LiDAR point clouds make self-driving cars vulnerable to spoofing attacks. We construct the first black-box spoofing attack based on our identified vulnerability, which universally achieves around 80% mean success rates on all target models. We perform the first defense study, proposing CARLO to mitigate LiDAR spoofing attacks. CARLO detects spoofed data by treating ignored occlusion patterns as invariant physical features, which reduces the mean attack success rate to 5.5%. Meanwhile, we take the first step towards exploring a general architecture for robust LiDAR-based perception, and propose SVF that embeds the neglected physical features into end-to-end learning. SVF further reduces the mean attack success rate to around 2.3%.

==> sections/Target.tex <==
\section{Target Perception Models and Benchmark}
\label{Target}

\subsection{Target Perception Models}
\label{target_models}

\begin{figure}[thp!]
\centering
  \missingfigure[figwidth=8cm]{Testing a long text string}
  \caption{Comparison with State-of-the-art LiDAR-based Perception Architectures.}
  \label{fig:sota}
  \vspace{-0.5cm}
\end{figure}

\subsubsection{Baidu Apollo 5.0 \footnote{\url{https://github.com/ApolloAuto/apollo/tree/r5.0.0/modules/perception/lidar}}}

Figure.\ref{fig:sota} (a) shows the perception pipelines of Apollo model

\subsubsection{PointPillars \footnote{\url{https://github.com/nutonomy/second.pytorch}}} Figure.\ref{fig:sota} (b) shows the perception pipelines of PointPillars model

\subsubsection{PointRCNN \footnote{\url{https://github.com/sshaoshuai/PointRCNN}}} 
Figure.\ref{fig:sota} (c) shows the perception pipelines of PointRCNN


\subsection{Target Benchmark}
\label{target_benchmark}

KITTI is 



==> sections/Vulnerability_old.tex <==
\section{A General Design-level Vulnerability}
\label{vulnerability}

% , among which 64-line LiDARs are particularly popular since they are not only cost-effective but can also ensure reliability while delivering the performance demanded by autonomous driving. \alfred{not sure whether this claim holds. Apollo is using 128-line lidar by default I think?} \mytodo{I will cite some articles for this} 

% Most AVs utilize high-resolution LiDAR sensors for safety enhancement, among which KITTI leverages Velodyne HDL-64Es for data collection (\S\ref{background_kitti})

As introduced in \S\ref{background_kitti}, a point cloud sample in KITTI consists of around 133,000 points, where a front-near vehicle should contain at least 2000 points and occupy about 15 $^\circ$ of horizontal angles\cite{Geiger2013IJRR}. However, Cao \etal demonstrated that an attack trace with 60 points and 8 $^\circ$ of horizontal angles is sufficient to spoof a front-near vehicle in Apollo 2.5\cite{cao2019adversarial}. It still remains unclear why such spoofing attacks can succeed even with a huge gap existing between adversarial and normal vehicles. Despite the promising results of attacking image-based machine learning models shown in previous studies\cite{eykholt2018robust,220580}, their approaches have internal differences with Adv-LiDAR. We distinguish the spoofing attacks towards LiDARs with extensive prior work in mainly three aspects: 

\textbf{Different perturbation methods.} Images and point clouds have different data structures, which further leads to different perturbation methods applied. Images have compact structures (\ie $H \times W \times C$), where $H \times W$ stands for the image size and $C$ contains the RGB information. However, point clouds are unordered which are oftentimes represented as $N \times C$, where $N$ is the number of points and $C$ contains the location and intensity information (\ie$xyz$-$i$). Attackers are able to generate adversarial examples by modifying the RGB values in images. For LiDAR-based attacks, however, attackers can directly shift the point in the 3D Euclidean space as long as it obeys the physics of LiDAR (\S\ref{background_direct_spoof}).

\textbf{Different perturbation capabilities.} Prior attacks towards 2D images always treat the whole target area as the attack surface since the threat models assumes that attackers have full controls over the target object (\eg the attackers can potentially modify any areas of a stop sign\cite{eykholt2018robust}). However, due to the characteristics of LiDAR spoofing attacks, the attack surface is limited by the sensor attack capability ($\mathcal{A}$) in \S\ref{threat}. Such a small attack surface also introduces more difficulties to launching the adversarial spoofing attack.

\textbf{Different perturbation constraints.} Prior attacks towards 2D images leverage \emph{l-p} norms as main constraints for the formulated optimization problem\cite{eykholt2018robust} whose goal is to minimize the perturbation to be stealthy. Such constraints are not applicable to attacking LiDAR because point clouds are not perceived by human beings, thus, stealthiness is not a focus in such attacks. However, due to the limited sensor attack capability (\S\ref{threat}), the optimized attack traces must not exceed the capability boundary, in which case the sensor attack capability naturally becomes the main constraint for attacking LiDAR.

Therefore, in order to unveil the general vulnerability exposed by Adv-LiDAR, it is necessary to take the distinct characteristics of the LiDAR point cloud into considerations, which are different from image-based attacks. %.... Table 1. summarize the notations we use in following subsections.  

% With so many differences, we hypothesize lies in the unique physical features of LiDAR point clouds. In the following sections, we first propose based on empirical observations and 

\subsection{Hypotheses Proposal}
\label{hypothesis}

\begin{figure}[thp!]
\centering
  \includegraphics[width=6cm]{images/C1-3.pdf}
  \caption{Illustration of \textbf{C1-3} of LiDAR point cloud.}
  \label{fig:c1-3}
\end{figure}

Although deep learning has been successfully applied to LiDAR-based object detection in autonomous driving, the interpretability of such models is always a bottleneck factor. In this section, we first provide several empirical observations (\textbf{O}) of LiDAR-based perception models and unique characteristics (\textbf{C}) of LiDAR point cloud data, based on what, we further propose two hypotheses (\textbf{H}) that could lead to a design-level vulnerability of state-of-the-art models.

\textbf{C1}: Occlusion between objects is inevitable in LiDAR point clouds and will cause partial visibility of the occluded objects. As introduced in \S\ref{background_spoof}, a LiDAR sensor functions by firing laser pulses and capturing their returns. As a result, each point in a point cloud represents the distance to the \emph{nearest} solid object that along the laser ray. Similar to human eyes, a LiDAR can only perceive parts of an object (\eg a vehicle) if other obstacles standing between the LiDAR and the object that exclude the laser beams. 

In this paper, we describe such occluded objects as \emph{occludees} and the objects that occlude others as \emph{occluders}. Particularly, we use $\mathsf{O}(x)$ to express the set of points that occludes the object $x$, and we use the captain letter $X$ to express the set of points that belong to object $x$ in the point cloud $F$ ($X = \{\vec{p}\, | \,\vec{p} \in x\} \subseteq F$, where $\vec{p} \in \mathbb{R}^3$).

\alfred{need a figure to illustrate the point} \mytodo{I will draw a figure to show C1-3}

\textbf{O1}: Deep learning identifies correlations in the training data, but it arguably cannot build causal models by purely observing correlations\cite{doshi2017towards}. The state-of-the-art LiDAR-based perception models (\S\ref{background}) most likely preserve this characteristic as they consist of basic fully-connected and convolutional layers.

\textbf{C2}: The \emph{occludee} and the corresponding \emph{occluders} described in \textbf{C1} stand separately from each other in the 3D Euclidean space. Intuitively, an occlusion relation exists as long as the \emph{occluders} shades the \emph{occludee} from the perspective of the LiDAR sensor As a result, $X$ and $\mathsf{O}(x)$ may be far apart with each other in the point cloud.

\textbf{O2}: CNNs exploit spatial locality by enforcing a local connectivity pattern between neurons of adjacent layers. The architecture thus ensures to produce the strongest response to a spatially local input pattern. PointPillars and Apollo 5.0 both leverage CNNs for the final detection task, so they are supposed to remain such characteristic, too. PointRCNN only accepts points inside region proposals into its second stage pipeline, thus spontaneously preserves locality. 

Occlusion is a causation relationship. The existence of the \emph{occluders} leads to the partial visibility of the corresponding \emph{occludee}. From \textbf{O1}, deep learning models can barely identify such causation relationship introduced by occlusions. Besides, since the $X$ and $\mathsf{O}(x)$ stand independently from each other in the 3D Euclidean space (\textbf{C2}), LiDAR-based perception models have limitations to even identify the correlation between the $X$ and $\mathsf{O}(x)$ due to \textbf{O2}. Thus, we propose our first hypothesis:   

\vspace{0.2cm}

\textbf{H1}: \emph{Given a point cloud $F$ containing an occluded object $x$, if $\mathcal{M}(F) \Rightarrow \{\mathsf{B}(x),\ldots\}$, we hypothesize $\mathcal{M}(F-\mathsf{O}(x)) \Rightarrow \{\mathsf{B}(x),\ldots\}$, where $\mathsf{B}(x)$ denotes the bounding box parameters of $x$.}

%\emph{The state-of-the-art LiDAR-based perception models have poor ability to learn the occlusion relationship in point clouds.}

\vspace{0.2cm}

\textbf{C3}: Due to the working principles of LiDAR sensors (\S\ref{spoof}), the generated point clouds are collected uniformly in vertical and horizontal angles but not in Euclidean space. The points farther away from the LiDAR sensor are generally sparser than the points nearby the sensor. The horizontal and vertical resolutions are  $\propto r\times\sin{\Delta \theta}$ and $\propto r\times\sin{\Delta \phi}$ respectively, where $r$ is the distance from the point to the LiDAR sensor, and $\Delta \theta$ and $\Delta \phi$ are the horizontal and vertical fire angle intervals.

\textbf{O3:} CNN-based 2D object detection models are oftentimes translation equivariant\cite{ren2015faster}. Intuitively, if an object is translated to another location in the image plane, its detected bounding box should shift with the translation of the original object\cite{weiler20183d}:
\begin{equation}
    \mathcal{M} \circ \mathsf{T}\,_{\vec{t}} = \mathsf{T}\,_{\vec{t}} \circ \mathcal{M}
\end{equation}
where $\mathsf{T}\,_{\vec{t}}(\vec{x}) := (\vec{x} + \vec{t})$, where $\vec{x},\vec{t} \in \mathbb{R}^2$ and $\mathcal{M}$ is the deep learning model. In terms of LiDAR-based perception models, first, the hard-coded features in the BEV-based models (\eg Apollo 5.0) do not contain location information in $xy$ plane, therefore, will most likely possess the characteristic in $xy$ plane. Second, for the voxel-based models, the initial features inside each voxel contain the location information (\ie $x,y,z$). However, they also incorporate the local location $x_c,y_c,z_c$ where the $c$ subscript denotes distance to the arithmetic mean of all points in the voxel (\S\ref{background}) which are translation equivariant. Thus, the characteristic may still hold in the voxel-based models. Third, in the second stage of the point-wise models, canonical coordination transformations are performed in each region proposal, regarding the centers of the region proposals as the origins of their coordinates. This canonical transformation automatically makes the model translation equivariant.

Even though the density of point clouds varies a lot along their distances to the sensor (\textbf{C3}), we propose our second hypothesis based on \textbf{O3}:

\vspace{0.2cm}

\textbf{H2}: \emph{Given a point cloud $F$ containing an object $x$, if $\mathcal{M}(F) \Rightarrow \{\mathsf{B}(x),\ldots\}$, we hypothesize $\mathcal{M}((F - X) \cup \mathsf{T}\,_{\vec{t}}(X)) \Rightarrow \{\mathsf{B}(\mathsf{T}\,_{\vec{t}}(x)),\ldots\}$, where $\mathsf{B}(x)$ denotes the bounding box parameters of $x$.}

%\emph{The state-of-the-art LiDAR-based perception models barely differentiate the detection results for the same set of points at different locations in the $xy$ plane.}

\subsection{Hypotheses Validation}
\label{hypothesis_validation}


We test the two proposed hypotheses using point clouds from the KITTI validation set. 

% As stated in \S\ref{threat}, we target vehicle detection in this paper. 

%Therefore, the designed experiments (\textbf{V}) also focus on vehicle detection. However, we believe both the experiments and results can be generalized to pedestrian and cyclist detection. 

\textbf{V1}: To validate \textbf{H1}, we first randomly pick 100 point cloud frames $\mathcal{F}=\{F_{i}\}_{i=1}^{100}$ that contain 100 target \emph{occluded} vehicles $\{v_{i}\}_{i=1}^{100}$ where the corresponding set of points $V_i \subseteq F_i$ respectively. We then feed $\mathcal{F}$ into three target models and record the confidence scores of the occluded vehicles as $s_i$ for each $v_i$. 

Second, we eliminate the specific $\mathsf{O}(v_i)$ for each vehicle $v_i$. The rest of points of each point cloud $F_{i}$ form a new set of point cloud frames $\mathcal{F}^{'}=\{F_{i}-\mathsf{O}(v_{i})\}_{i=1}^{100}$. We feed $\mathcal{F}^{'}$ into the three target models and record new confidence scores of the occluded vehicles as ${s_i}'$ for each $v_i$. 

Figure \ref{fig:cdf} shows the CDF of $e = \frac{|{s_i}'-{s_i}|}{{s_i}}$ for all three target models. As shown, 99.5\% of the picked occluded vehicles only have below 2\% fluctuations of their confidence scores when their corresponding $\mathsf{O}(\cdot)$ are eliminated from the point cloud on all target models. The experimental results validate \textbf{H1}. 

\textbf{V2}: To validate \textbf{H2}, we first generate a point cloud $G$ simulating the ground plane's points as reference for the $xy$ plane. Then we again randomly pick and extract 100 vehicles' point clouds $\mathcal{V}=\{V_{i}\}_{i=1}^{100}$. It is worth noting that they are not necessary occluded. We further merge the point cloud of the ground plane $G$ with $\mathcal{V}$ forming a new set $\mathcal{F}=\{G \cup V_{i}\}_{i=1}^{100}$. We feed $\mathcal{F}$ into three target models and record the confidence scores of the occluded vehicles as $s_i$ for each $v_i$.

Second, we grid the ground plane $G$ into 1 $m^2$ cells $\{(x_{p},y_{q})\}_{p,q=1}^{N_{x},N_{y}}$, where $N_{x}$ and $N_{y}$ are the number of cells in $x$ and $y$ axes respectively. By applying a global transformation matrix $H(\theta,\tau)$\cite{cao2019adversarial} to $\mathcal{V}$, we translate every $V_{i}$ to every cell $(x_{p},y_{q})$ on the ground plane as $V_{i,p,q}'$:
\begin{equation}
\begin{split}
& \quad {V_{i,p,q}'}_{\wi} = {V_{i}}_{\wi} \\
\begin{bmatrix}
  {V_{i,p,q}'}_{\wx}\\
  {V_{i,p,q}'}_{\wy}\\
  {V_{i,p,q}'}_{\wz}\\
  1 
\end{bmatrix} & = \begin{bmatrix}
  \cos{\theta} & -\sin{\theta} & 0 & \tau\cos{\theta}\\
  \sin{\theta} & \cos{\theta} & 0 & \tau\sin{\theta}\\
  0 & 0 & 1 & 0 \\
  0 & 0 & 0 & 1 \\
\end{bmatrix} 
\cdot 
\begin{bmatrix}
  {V_{i}}_{\wx}\\
  {V_{i}}_{\wy}\\
  {V_{i}}_{\wz}\\
  1
\end{bmatrix}
\end{split}
\end{equation}
where $({V_{i}}_{\wx},{V_{i}}_{\wy},{V_{i}}_{\wz},{V_{i}}_{\wi})$ denotes the $xyz$-$i$ features of all points in $V_{i}$. We merge the $V_{i,p,q}'$ with $G$ forming $\mathcal{F}'=\{V_{i,p,q}' \cup G\}_{i,p,q=1}^{100,N_{x},N_{y}}$. We feed $\mathcal{F}'$ into three target models and record the confidence score of the translated vehicle as $s_{i,p,q}'$. 

Figure \ref{fig:cdf} also shows the CDF of $e' = \frac{|s_{i,p,q}'-{s_i}|}{{s_i}}$ for all three target models. As shown, the relative error $e'$ are larger than $e$, which is expected since the models contain location-sensitive features (\textbf{O3}). However, the results the fluctuations are still below 10\% for 99.5\% picked vehicles, and we verify that with such fluctuations, the models still detect these vehicles as valid which validate \textbf{H2}.

\begin{figure}[thp!]
\centering
  \includegraphics[width=1\linewidth, height=0.4\linewidth]{images/cdf.pdf}
  \caption{CDF of the relative errors $e$ (left) and $e'$ (right).}
  \label{fig:cdf}
  \vspace{-0.5cm}
\end{figure}


\subsection{Vulnerability Identification}
\label{vulnerability_id}

In this section, we unveil how the validated hypotheses (\textbf{V1-2}) lead to a design-level vulnerability of state-of-the-art LiDAR-based perception models. 

As introduced in \S\ref{background_adv_spoof}, Equation \ref{eq:adv_lidar} formulates the optimization problem of the adversarial spoofing attack, where $\mathcal{A}$ is the sensor attack capability. 
%We adopt the formulation of sensor attack capability in \cite{cao2019adversarial}(\S\ref{threat}), and in our reproduced sensor attack, the number of spoofed points is limited to 200 points and the horizontal angle is limited to 10 $^\circ$. The capability is far from spoofing a complete vehicle's point cloud. 

Instead of spoofing a complete vehicle, to spoof an occluded vehicle is a much easier task since an occluded vehicle occupies smaller horizontal angles and less points than a complete one. \textbf{V1} shows that even without a valid \emph{occluder}, an ``occluded'' vehicle can still be detected by the models. Moreover, attackers can spoof even sparser points of an occluded vehicle to further reduce the cost. Due to the non-uniform density of LiDAR point clouds (\textbf{C3}), a vehicle far away from the LiDAR sensor contains sparse points. \textbf{V2} shows that translating such a distant vehicle's points to a nearby location will make the models detect the translated points as a vehicle at the new location. 

As a result, instead of formulating the $\oplus$ function and solving Equation \ref{eq:adv_lidar} by gradient descent-based methods, attackers can directly spoof an ``occluded'' vehicle with sparse points that satisfy the sensor attack capability $\mathcal{A}$ to fool the state-of-the-art models. \mytodo{not sure whether the explanation is clear.}
